GenAI Content Detection Task 1: English and Multilingual Machine-Generated Text Detection: AI vs. Human

We present the GenAI Content Detection Task~1 -- a shared task on binary machine generated text detection, conducted as a part of the GenAI workshop at COLING 2025. The task consists of two subtasks: Monolingual (English) and Multilingual. The shared task attracted many participants: 36 teams made official submissions to the Monolingual subtask during the test phase and 26 teams -- to the Multilingual. We provide a comprehensive overview of the data, a summary of the results -- including system rankings and performance scores -- detailed descriptions of the participating systems, and an in-depth analysis of submissions. https://github.com/mbzuai-nlp/COLING-2025-Workshop-on-MGT-Detection-Task1

==> section/9_rank_results.tex <==
\section{Participants' Submissions}
In this section, we first describe ranking, macro-F1 and accuracy of participants, followed by a brief description of all submitted systems.
We classify methods into (1) above vs. below the baseline, (2) black-box vs. white-box, (3) zero-shot vs. fine-tuning, (4) fine-tuning based on small models vs. large models, and (5) ensemble or not. 

\subsection{English Results and Rank}

% \subsubsection{Results and Rank}
\input{tables/results_en}

The English subtask attracted 36 submissions in total. \autoref{tab:results_en} presents the complete rankings. The competition saw a remarkably tight race among the top performers with only 0.27 macro-F1 points separating the top three teams: ``Advacheck'' (83.07), ``Unibuc-NLP'' (83.01), and ``Fraunhofer SIT'' (82.8). Interestingly, while the team ``Advacheck'' secured the first place by the main metric, ``Unibuc-NLP'' achieved a slightly higher accuracy (83.33 vs. 83.11), highlighting the razor-thin margins between top performers.

Fourteen teams outperformed the baseline (73.42 macro-F1) according to the main metric with overall scores varying from 83.07 to 44.89. The inability of most submissions to surpass the baseline underscores the complexity of the task.


\subsection{Multilingual Results and Ranks}

% \subsubsection{Results and Ranks}

\input{tables/results_multi}

The multilingual subtask received 27 submissions with complete rankings demonstrated in \autoref{tab:results_multi}.

The most notable feature of this subtask was the exceptional performance of the team ``Grape'', achieving macro-F1 score of 79.16, significantly outperforming other competitors. A substantial gap of 3.59 macro-F1 points between the winner and the second place ``rockstart'' (75.57) underscores the effectiveness of the ``Grape'' team approach to multilingual MGT detection.

In this subtask, only seven teams managed to surpass the baseline score of 74.16 with scores ranging from 79.16 to 51.03. This indicates the increased difficulty of detecting MGT text among multiple languages simultaneously.

The overall lower scores in this subtask compared to the English subtask (top score 79.16 vs. 83.07) highlight the additional complexity introduced by multilingual detection and room for improvement. 
%This finding may suggest that although current approaches work reasonably well for single-language detection, there is still room for improvement in multilingual scenarios.



==> section/9_system_description.tex <==
\subsection{Mononlingual System Description}
\input{tables/systems_en}
\autoref{tab:systems_en} presents an overview of the English subtask participants' systems. 

\noindent \textbf{Team Advacheck$_{\text{English:1}}$} \cite{genai-detect:2025:task:Advacheck} develops a multi-task system with a shared Transformer Encoder (DeBERTa-v3-base) between several classification heads. This system includes a primary binary classification head and additional multiclass heads for text domain classification. The ablation studies show that multi-task learning outperforms single-task modes, with simultaneous tasks forming cluster structures in the embeddings space.

\noindent \textbf{Team Unibuc-NLP$_{\text{English:2}}$} \cite{genai-detect:2025:task:UnibucNLP} utilized both masked (XLM-RoBERTa-base) and causal language models (Qwen2.5-0.5B; \citealp{qwen2.5}), with the Qwen-based classifier performing on par with \citeauthor{genai-detect:2025:task:Advacheck}. The authors report that LORA fine-tuning XLM-RoBERTa promotes a strong performance. 

\noindent \textbf{Team Fraunhofer SIT$_{\text{English:3}}$} \cite{genai-detect:2025:task:FraunhoferSIT} combined an MGT detection adapter with a multi-genre natural language inference adapter over RoBERTa-base. 
%This system earned the third place.

\noindent \textbf{Team Grape$_{\text{English:4}}$} \cite{genai-detect:2025:task:Grape}, first,
%took the fourth place. First, the authors 
finetuned Llama-3.2-1B \cite{dubey2024llama} and gemma-2-2b \cite{team2024gemma} for the MGT detection task. Second, they combined linguistic features with the model predictions by leveraging ensemble learning for more robust classification.

\noindent \textbf{Team TechExperts(IPN)$_{\text{English:5}}$} 
%was ranked fifth in the leaderboard. 
similar to \citeauthor{genai-detect:2025:task:Grape} fine-tuned gemma-2b for the MGT detection task, which confirms the effectiveness of the small model in identifying the generated content.

\noindent \textbf{Other teams} ranked in top-20 developed the MGT detectors by (i) fine-tuning a model (\textbf{Team TurQUaz$_{\text{English:6}}$}; \citealp{genai-detect:2025:task:TurQUaz};  \textbf{Team AAIG$_{\text{English:8}}$}; \citealp{genai-detect:2025:task:AAIG}; \textbf{Team IPN-CIC$_{\text{English:18}}$}; \citealp{genai-detect:2025:task:abit7431}; \textbf{Team Ai-Monitors$_{\text{English:19}}$}; \citealp{genai-detect:2025:task:AI-Monitors}); (ii) ensembling models and features (\textbf{Team SzegedAI$_{\text{English:7}}$}; \citealp{genai-detect:2025:task:SzegedAI}; \textbf{Team DCBU$_{\text{English:9}}$}; \citealp{genai-detect:2025:task:dcbu}; \textbf{Team Lux Veri$_{\text{English:12}}$}; \citealp{genai-detect:2025:task:LuxVeri}); and (ii) utilizing label supervision (\textbf{Team L3i++$_{\text{English:11}}$}; \citealp{genai-detect:2025:task:L3i++}).




\subsection{Multilingual System Description}
%: Rui
\input{tables/systems_multi}

\autoref{tab:systems_multi} presents an overview of the multilingual subtask participants' systems. 
% team rank and system description status

% rank 1 nhidaon
\noindent \textbf{Team Grape$_{\text{Multi:1}}$}~\citep{genai-detect:2025:task:Grape}, ranked 1 in the multilingual leaderboard, adopted two approaches in the task. They first separately fine-tuned small language models tailored to the specific subtask. Then they built on the first step by incorporating linguistic, syntactic and semantic features, leveraging ensemble learning to integrate these features with model predictions for more robust classification. Through evaluating and comparing these approaches, the team identified the most effective techniques for detecting machine-generated content across languages.

% rank 2 rockstart NO system desc

% rank 3 hancheolp
\noindent \textbf{Team NotaAI$_{\text{Multi:3}}$}~\citep{genai-detect:2025:task:NotaAI} secured the third place in the task. They developed the system that addresses the challenge of detecting MGT in languages not observed during training, where model accuracy tends to decline significantly. The proposed multilingual MGT detection system employs a two-step approach: first, a language identification tool determines the language of the input text. If the language has been observed during training, the text is processed using a model fine-tuned on a multilingual PLM. For languages not seen during training, the system utilizes a model that combines token-level predictive distributions extracted from various LLMs with a meaning representation derived from a multilingual PLM.

% rank 4 mobin
\noindent \textbf{Team LuxVeri$_{\text{Multi:4}}$}~\citep{genai-detect:2025:task:LuxVeri} earned the 4th place. They utilized an ensemble of models, where weights are assigned based on each model's inverse perplexity to improve classification accuracy. The system combined RemBERT, XLM-RoBERTa-base, and BERT-base-multilingual-cased using the same weighted ensemble strategy. The results highlight the effectiveness of inverse perplexity-based weighting for robust detection of machine-generated text in both monolingual and multilingual settings.

% rank 5 LACKING details of system desc
\noindent \textbf{Team TecExperts(IPN)$_{\text{Multi:5}}$}~\citep{genai-detect:2025:task:TecExperts(IPN)} leveraged the gemma-2b model, fine-tuned specifically for the Shared Task 1 datasets to achieve strong performance.

% rank 6 NO system desc

% rank 7 nampfiev1995
\noindent \textbf{Team L3i++$_{\text{Multi:7}}$}~\citep{genai-detect:2025:task:L3i++} studied a label-supervised adaptation configuration for LLaMA-as-a-judge for the task. In detail, they explore the feasibility of fine-tuning LLaMA with label supervision in masked and unmasked, unidirectional and bidirectional settings, to discriminate the texts generated by machines and humans in monolingual and multilingual corpora.


% other systems below baselines
\noindent \textbf{Other Systems} The other systems explored various approaches, including exploring the integration of additional features such as perplexity and Tf-IDF~(\textbf{Team TurQUaz$_{\text{Multi:22}}$};~\citealp{genai-detect:2025:task:TurQUaz}), finetuning models such as XLM-RoBERTa on the training set for the final evaluation, as incorporating adapter fusion led to worse results~(\textbf{Team Fraunhofer SIT$_{\text{Multi:10}}$};~\citealp{genai-detect:2025:task:FraunhoferSIT}), XML-R and mBERT models~(\textbf{Team IPN$_{\text{Multi:9}}$};~\citealp{genai-detect:2025:task:abit7431} and QWen and RoBERTa models~(\textbf{Team Unibuc-NLP$_{\text{Multi:22}}$};~\citealp{genai-detect:2025:task:UnibucNLP}); and combining language-specific embeddings with fusion techniques to create a unified, language-agnostic feature representation~(\textbf{Team OSINT$_{\text{Multi:15}}$};~\citealp{genai-detect:2025:task:OSINT}).

% rank 9 abit7431 LACKING details described in other systems

% rank 10 karla FraunhoferSIT described in other systems

% rank 15 Shifali OSINT described in other systems

% rank 22- keles described in other systems



==> tables/analysis_tables_2f.tex <==
\begin{table}[t!]
    \centering
    \small
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{cccccc}
    \toprule
    \textbf{Rank} & \textbf{All} & \textbf{MixSet} & \textbf{CUDRT} & \textbf{IELTS} & \textbf{PeerReview} \\
    \midrule
    1 & 83.11 & 48.02 & 67.12 & 89.90 & 97.25 \\
    2 & 83.33 & 66.72 & 75.93 & 82.62 & 94.10 \\
    3 & 82.89 & 58.92 & 70.99 & 88.82 & 92.13 \\
    4 & 82.23 & 64.69 & 73.24 & 79.14 & 97.35 \\
    5 & 81.81 & 59.21 & 72.67 & 80.85 & 95.53 \\
    6 & 80.74 & 47.25 & 72.61 & 78.11 & 96.92 \\
    7 & 75.68 & 54.85 & 71.04 & 63.11 & 97.19 \\
    8 & 79.34 & 62.31 & 75.42 & 68.96 & 97.16 \\
    9 & 78.01 & 59.95 & 74.60 & 66.31 & 96.92 \\
    10 & 76.42 & 59.84 & 75.52 & 64.17 & 93.16 \\
    11 & 75.54 & 60.93 & 70.28 & 66.86 & 92.50 \\
    12 & 75.68 & 56.63 & 74.00 & 61.94 & 95.20 \\
    13 & 75.17 & 62.77 & 70.79 & 65.33 & 92.16 \\
    14 & 75.14 & 66.58 & 72.84 & 62.71 & 92.23 \\
    \hdashline 
    Baseline & 74.89 & 61.99 & 72.12 & 63.36 & 92.17 \\
    \hdashline 
    15 & 74.83 & 73.21 & 71.91 & 63.03 & 90.81 \\
    - & 73.16 & 53.53 & 71.30 & 62.79 & 89.30 \\
    16 & 73.89 & 64.34 & 71.24 & 62.58 & 90.28 \\
    17 & 71.42 & 53.93 & 69.62 & 70.83 & 76.57 \\
    18 & 72.42 & 65.40 & 70.61 & 62.17 & 86.45 \\
    19 & 72.65 & 72.63 & 70.38 & 63.59 & 84.77 \\
    20 & 71.96 & 69.76 & 70.37 & 66.53 & 79.79 \\
    21 & 69.51 & 50.75 & 63.98 & 65.74 & 82.04 \\
    22 & 70.50 & 70.63 & 66.71 & 65.30 & 79.95 \\
    23 & 68.76 & 73.69 & 66.89 & 61.66 & 77.59 \\
    24 & 68.46 & 65.69 & 67.33 & 57.42 & 81.99 \\
    25 & 67.48 & 67.56 & 67.71 & 57.97 & 77.53 \\
    26 & 67.25 & 68.22 & 67.20 & 57.26 & 77.99 \\
    27 & 66.69 & 67.41 & 67.10 & 57.13 & 76.53 \\
    28 & 63.20 & 68.30 & 67.84 & 57.06 & 64.40 \\
    29 & 63.49 & 67.67 & 68.59 & 57.64 & 64.05 \\
    30 & 64.20 & 77.68 & 64.45 & 58.62 & 67.93 \\
    31 & 60.37 & 77.74 & 64.64 & 58.31 & 55.65 \\
    32 & 50.78 & 55.97 & 49.70 & 51.10 & 50.73 \\
    33 & 50.60 & 56.71 & 49.14 & 50.68 & 51.05 \\
    34 & 56.65 & 80.75 & 60.61 & 54.89 & 50.88 \\
    35 & 57.24 & 82.27 & 56.36 & 54.00 & 57.81 \\
    \bottomrule
    \end{tabular}
}
    \caption{\textbf{English Subtask detection accuracy} across four datasets or domains.}
    \label{tab:ana-english-domain-impact}
\end{table}



\begin{table*}[t]
    \centering
    % \small
     \scriptsize
    % \resizebox{\textwidth}{!}{
    \begin{tabular}{cccccccccc}
    \toprule
    \textbf{Rank} & \textbf{All} & \textbf{News} & \textbf{Wikipedia} & \textbf{Essay} & \textbf{QA} & \textbf{Summary} & \textbf{Tweet} & \textbf{GovReport} &\textbf{ Other} \\
    Size & 151,425 & 57,590 & 11,687 & 2,201 & 24,854 & 13,600 & 1,325 & 19,736 & 4,214 \\
    \midrule
    \textbf{Baseline} & 74.75 & 61.58 & 85.24 & 97.68 & 94.09 & 58.60 & 94.42 & 76.16 & 83.20 \\
    1 & 79.62 & 65.12 & 80.16 & 99.32 & 98.93 & 69.99 & 94.49 & 86.99 & 84.15 \\
    2 & 75.64 & 64.05 & 87.06 & 81.01 & 91.86 & 79.12 & 100.00 & 69.12 & 48.17 \\
    3 & 75.91 & 60.71 & 81.02 & 97.73 & 96.15 & 65.21 & 72.00 & 81.72 & 91.10 \\
    4 & 75.27 & 60.67 & 87.93 & 91.00 & 93.16 & 71.72 & 98.94 & 75.16 & 58.64 \\
    5 & 74.74 & 60.19 & 74.69 & 97.68 & 98.90 & 59.73 & 65.28 & 74.98 & 96.23 \\
    6 & 74.49 & 59.81 & 79.63 & 90.87 & 95.09 & 82.77 & 95.47 & 62.59 & 82.65 \\
    7 & 74.40 & 59.81 & 79.73 & 90.73 & 95.24 & 82.07 & 93.81 & 62.90 & 79.38 \\
    8 & 73.92 & 58.08 & 81.25 & 98.46 & 92.93 & 73.48 & 29.06 & 81.21 & 70.72 \\
    9 & 73.48 & 61.11 & 85.03 & 94.73 & 94.55 & 64.83 & 87.85 & 78.69 & 60.30 \\
    10 & 73.61 & 60.82 & 77.33 & 94.18 & 95.42 & 61.32 & 91.92 & 80.51 & 86.81 \\
    11 & 73.34 & 60.15 & 83.93 & 96.68 & 94.93 & 60.04 & 56.00 & 82.38 & 61.84 \\
    12 & 73.52 & 62.19 & 81.40 & 93.32 & 95.87 & 64.79 & 40.98 & 83.55 & 68.25 \\
    13 & 72.00 & 56.29 & 42.31 & 99.23 & 99.22 & 70.93 & 33.74 & 89.00 & 67.32 \\
    14 & 70.99 & 55.96 & 55.20 & 97.05 & 92.36 & 76.26 & 0.08 & 81.07 & 85.64 \\
    15 & 50.35 & 51.04 & 42.41 & 60.02 & 51.20 & 49.68 & 33.89 & 61.91 & 62.13 \\
    16 & 71.51 & 59.60 & 43.97 & 97.05 & 99.16 & 59.50 & 57.66 & 89.26 & 58.14 \\
    17 & 50.21 & 50.81 & 43.18 & 57.66 & 50.75 & 49.90 & 36.60 & 59.83 & 60.80 \\
    18 & 69.63 & 55.01 & 45.76 & 97.73 & 92.23 & 71.47 & 2.34 & 82.74 & 85.22 \\
    19 & 70.47 & 54.55 & 33.53 & 99.14 & 99.14 & 73.12 & 6.42 & 88.73 & 77.57 \\
    20 & 70.65 & 60.89 & 41.72 & 93.46 & 99.14 & 63.52 & 45.28 & 86.84 & 61.34 \\
    21 & 67.91 & 61.72 & 69.89 & 63.56 & 78.11 & 78.03 & 49.36 & 71.77 & 60.68 \\
    22 & 67.11 & 57.36 & 51.77 & 83.42 & 94.67 & 61.54 & 100.00 & 80.70 & 20.88 \\
    23 & 49.71 & 49.08 & 57.00 & 45.52 & 49.11 & 50.26 & 64.45 & 40.07 & 39.42 \\
    24 & 52.59 & 45.33 & 35.01 & 82.96 & 72.38 & 67.30 & 99.32 & 46.64 & 17.75 \\
    25 & 51.05 & 50.36 & 53.02 & 50.98 & 51.77 & 52.03 & 56.15 & 48.36 & 48.88 \\
    \bottomrule
    \end{tabular}
% }
    \caption{\textbf{Multilingual subtask detection accuracy} across eight domains.}
    \label{tab:ana-multilingual-domain-impact}
\end{table*}



\begin{table}[t!]
    \centering
    % \scriptsize
    \small
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{ccccc}
    \toprule
    \textbf{Rank} & \textbf{All} & \textbf{Fill-gap} & \textbf{Original} & \textbf{Others}\\
    Size & 151,425 & 32,487 & 17,017 &  101,921 \\
    \midrule
    1 & 79.62 & 91.09 & 94.15 & 73.53 \\
    2 & 75.64 & 75.94 & 84.00 & 74.14 \\
    3 & 75.91 & 89.74 & 92.24 & 68.78 \\
    4 & 75.27 & 81.49 & 86.90 & 71.35 \\
    \hdashline 
    \textbf{Baseline} & 74.75 & 87.61 & 89.05 & 68.26 \\
    \hdashline
    5 & 74.74 & 84.64 & 96.61 & 67.94 \\
    6 & 74.49 & 75.61 & 90.14 & 71.53 \\
    7 & 74.40 & 75.43 & 90.34 & 71.41 \\
    8 & 73.92 & 88.55 & 87.08 & 67.05 \\
    9 & 73.48 & 86.67 & 93.11 & 66.01 \\
    10 & 73.61 & 92.86 & 93.02 & 64.23 \\
    11 & 73.34 & 88.28 & 91.64 & 65.53 \\
    12 & 73.52 & 91.62 & 94.31 & 64.27 \\
    13 & 72.00 & 93.70 & 95.68 & 61.14 \\
    14 & 70.99 & 90.39 & 86.30 & 62.25 \\
    15 & 50.35 & 66.72 & 64.84 & 42.72 \\
    16 & 71.51 & 93.22 & 96.43 & 60.42 \\
    17 & 50.21 & 64.68 & 62.88 & 43.48 \\
    18 & 69.63 & 91.63 & 86.50 & 59.80 \\
    19 & 70.47 & 94.94 & 95.09 & 58.56 \\
    20 & 70.65 & 93.79 & 96.13 & 59.03 \\
    21 & 67.91 & 79.92 & 71.53 & 63.48 \\
    22 & 67.11 & 84.64 & 94.36 & 56.97 \\
    23 & 49.71 & 36.13 & 37.36 & 56.10 \\
    24 & 52.59 & 66.44 & 60.33 & 46.89 \\
    25 & 51.05 & 48.20 & 48.55 & 52.38 \\
    \bottomrule
    \end{tabular}
}
    \caption{\textbf{Multilingual subtask detection accuracy} between generations using original prompts vs. prompts aiming to fill the gap between human and machine, corresponding to columns of \textit{Original} vs. \textit{Fill-gap}. All is the whole multilingual test set.}
    \label{tab:ana-prompt-impact}
\end{table}
